The ART of Sharing Points-to Analysis (Extended Abstract)

Data-flow analyses like points-to analysis can vastly improve the precision of other analyses, and help perform powerful code optimizations. However, whole-program points-to analysis of large programs tend to be expensive - both in terms of time and memory. Consequently, many compilers (both static and JIT) and program-analysis tools tend to employ faster - but more conservative - points-to analysis to improve usability. As an alternative to such trading of precision for performance, various techniques have been proposed to perform precise yet expensive fixed-point points-to analyses ahead of time in a static analyzer, store the results, and then transmit them to independent compilation/program-analysis stages that may need them. However, an underlying concern of safety affects all such techniques - can a compiler (or program analysis tool) trust the points-to analysis results generated by another compiler/tool? In this work, we address this issue of trust, while keeping the issues of performance efficiency in mind. We propose ART: Analysis-results Representation Template - a novel scheme to efficiently and concisely encode results of flow-sensitive, context-insensitive points-to analysis computed by a static analyzer for use in any independent system that may benefit from such a highly precise points-to analysis. Our scheme has two components: (i) a producer that can statically perform expensive points-to analysis and encode the same concisely. (ii) a consumer that, on receiving such encoded results, can regenerate the points-to analysis results encoded by the artwork if it is deemed safe. We demonstrate the usage of ART by implementing a producer (in Soot) and two consumers (in Soot and the Eclipse OpenJ9 JIT compiler). We evaluate our implementation over various benchmarks from the DaCapo and SPECjvm2008 suites.

==> algos/jitc-algo-inter.tex <==
\SetKwProg{Fn}{Function}{}{end}
\SetKwProg{macro}{Macro}{}{end}
\SetKwFunction{make}{makeInterProcEASY}%
\SetKwFunction{topo}{topologicalSortCFG}%
\SetKwFunction{nE}{notEmpty}%
\SetKwFunction{pop}{pop}%
\SetKwFunction{artExists}{ARTExists}%
\SetKwFunction{getART}{getART}%
\SetKwFunction{trans}{transferFunction}%
\SetKwFunction{loopVer}{loopInvariantVerify}%
\SetKwFunction{outVer}{outInvariantVerify}%
\SetKwFunction{callsiteVer}{inInvariantVerify}%
\SetKwFunction{succ}{successors}%
\SetKwFunction{isCallsite}{isCallsite}%
\SetKwFunction{isNonRecCallsite}{isNonRecursiveCallsite}%
\SetKwFunction{isRecCallsite}{isRecursiveCallsite}%
\SetKwFunction{getCallee}{getCallee}%
\SetKwFunction{getCallees}{getCallees}%
\SetKwInOut{Input}{input}
\SetKw{false}{false}
\SetKw{true}{true}
\SetKw{assert}{assert}
\SetKwInOut{Output}{output}
\SetAlgoNoEnd


\begin{algorithm}[H]
	\small
\begin{multicols}{2}

  \Fn{\make{m, in}}{
    %\Input{ $m:$ method to be analyzed \\ $in:$ in-flow}
    %\Output{$PTA$ for $m$}
    $\text{IN[entry]} \gets in$\;
    $\text{recursiveOutUsed} \gets \false$\;
    $\text{analyzed[*]} \gets \false$\;
    $\mathcal{W} \gets \topo{m}$\;
    \While{\nE{$\mathcal{W}$}} { 
      $\text{l} \gets \mathcal{W}.\pop{}$\;
      \If{\isNonRecCallsite{l}}{
	\ForEach{c $\in$ \getCallees{l}} {
	  \callsiteVer{c, IN[l]}\;
	  $\text{in-flow} \gets \getART{l}$\;
	  $\text{callee-out} \gets \make{\getCallee{l},  in-flow}$\;
	}
      }
      \Else {
	    $\mathcal{A} \gets \getART{l}$\;
	\If{$\mathcal{A} \neq \phi$} {
	  OUT[l] $\gets \mathcal{A}$\;
	}
	\Else {
	  OUT[l] $\gets \trans{l}$\;
	}
	analyzed[l] $\gets \true$\;
	\ForEach{succ $\in$ \succ{l}} { 
	  \If{analyzed[succ]} {
		\loopVer{succ, l}\;
	  }
	}
      }
    }
    \If{recursiveOutUsed} {
	    \outVer{m, OUT}\;
    }

    \KwRet OUT\;
  }
\BlankLine
\BlankLine
\BlankLine
\macro{\getCallees{l}} {
\SetNoFillComment
  \tcc{resolve callee methods at callsite}
}

\BlankLine
\BlankLine
\BlankLine
\Fn{\loopVer{succ, l}}{
  \assert $\mathcal{I}_{loop}[l] \supseteq_s \text{IN[l]} \sqcap \text{OUT[succ]}$\;
}
\BlankLine
\BlankLine
\BlankLine
\Fn{\outVer{m, OUT}}{
  \assert $\mathcal{I}_{out}[m] \supseteq_s \text{OUT[m]}$\;
}
\BlankLine
\BlankLine
\BlankLine
\Fn{\getART{l}}{
  \If{\isRecCallsite{l}} {
    recursiveOutUsed $\gets \true$\;
    \KwRet $\mathcal{I}_{out}[\getCallee{l}]$\;
  }
  \ElseIf{\isNonRecCallsite{l}} {
    \KwRet $\mathcal{I}_{in}[\getCallee{l}]$\;
  }
  \Else {
    \KwRet $\mathcal{I}_{loop}[l]$\;
  }
}

\BlankLine
\BlankLine
\BlankLine
\macro{\trans{l}}{
\SetNoFillComment
  \tcc{apply relevant points-to analysis transfer function and return OUT[l]}
}

\end{multicols}
\end{algorithm}


==> algos/jitc-algo-intra.tex <==
\SetKwProg{Fn}{Function}{}{end}
\SetKwProg{macro}{Macro}{}{end}
\SetKwFunction{make}{makeEASY}%
\SetKwFunction{topo}{topologicalSortCFG}%
\SetKwFunction{nE}{notEmpty}%
\SetKwFunction{pop}{pop}%
\SetKwFunction{artExists}{ARTExists}%
\SetKwFunction{getART}{getART}%
\SetKwFunction{trans}{transferFunction}%
\SetKwFunction{loopVer}{loopInvariantVerify}%
\SetKwFunction{outVer}{outInvariantVerify}%
\SetKwFunction{succ}{successors}%
\SetKwFunction{isRecCallsite}{isRecursiveCallsite}%
\SetKwFunction{getCallee}{getCallee}%
\SetKwInOut{Input}{input}
\SetKw{false}{false}
\SetKw{true}{true}
\SetKw{assert}{assert}
\SetKwInOut{Output}{output}
\SetAlgoNoEnd
\begin{algorithm}[H]
	\small
\begin{multicols}{2}
\Fn{\make{m, in}}{
%\Input{ $m:$ method to be analyzed \\ $in:$ in-flow}
%\Output{$PTA$ for $m$}
  $\text{IN[entry]} \gets in$\;
  $\text{recursiveOutUsed} \gets \false$\;
  $\text{analyzed[*]} \gets \false$\;
$\mathcal{W} \gets \topo{m}$\;
\While{\nE{$\mathcal{W}$}} { 
  $\text{l} \gets \mathcal{W}.\pop{}$\;
$\mathcal{A} \gets \getART{l}$\;
\If{$\mathcal{A} \neq \phi$} {
OUT[l] $\gets \mathcal{A}$\;
}
\Else {
OUT[l] $\gets \trans{l}$\;
}
analyzed[l] $\gets \true$\;
\ForEach{succ $\in$ \succ{l}} { 
  \If{analyzed[succ]} {
	\loopVer{succ, l}\;
}
}
}
\If{recursiveOutUsed} {
	\outVer{m, OUT}\;
}

\KwRet OUT\;
}
\BlankLine
\BlankLine
\BlankLine
\Fn{\loopVer{succ, l}}{
  \assert $\mathcal{I}_{loop}[l] \supseteq_s \text{IN[l]} \sqcap \text{OUT[succ]}$\;
}
\BlankLine
\BlankLine
\BlankLine
\Fn{\outVer{m, OUT}}{
  \assert $\mathcal{I}_{out}[m] \supseteq_s \text{OUT[m]}$\;
}
\BlankLine
\BlankLine
\BlankLine
\Fn{\getART{l}}{
\If{\isRecCallsite{l}} {
recursiveOutUsed $\gets \true$\;
\KwRet $\mathcal{I}_{out}[\getCallee{l}]$\;
}
\Else {
\KwRet $\mathcal{I}_{loop}[l]$\;
}
}

\BlankLine
\BlankLine
\BlankLine
\macro{\trans{l}}{
\SetNoFillComment
\tcc{apply relevant points-to analysis transfer function and return OUT[l]}
}

\end{multicols}
\end{algorithm}


==> diagrams/art-composition.tex <==

	\[
		ART(PTA)   
		\begin{cases}
			\mathcal{I}_{loop} : l \rightarrow G, \forall l \in \text{loop-headers}
			\\ \\
			\mathcal{I}_{out} : M \rightarrow G, \forall M \in \text{recursive-methods}
			\\ \\
			\mathcal{I}_{in} : M \rightarrow G, \forall M \in \text{methods}
		\end{cases}
	\]


==> diagrams/art-intra-regen-consumer.tex <==
\begin{tabular}{l}
	\small
	$\out{{\tt Entry}} \gets \bot$ \\\\
	$\out{s_2} \gets f_2(\out{{\tt entry}})$ \\\\
	$\out{s_3} \gets f_3(\out{s_2})$ \\\\
	$\out{s_4} \gets f_4(\out{s_3})$ \\\\
	$\out{s_5} \gets f_5(\out{s_4})$ \\\\
	$\out{s_6} \gets f_6(\out{s_5})$ \\\\
	$\out{s_7} \gets f_7(\out{s_6})$ \\\\
	$\out{s_8} \gets f_8(\iloop[s_8])$ \\\\
	$\out{s_9} \gets f_9(\out{s_8})$ \\\\
	$\out{s_{10}} \gets f_{10}(\out{s_9})$ \\\\
	$\out{s_{12}} \gets f_{12}(\out{s_8})$ \\\\
	$\out{{\tt Exit}} \gets \out{s_{12}}$ \\
\end{tabular}


==> diagrams/art-intra-regen-producer.tex <==
\begin{tabular}{l}
	\small
	$\out{{\tt Entry}} \gets \bot$ \\\\
	$\out{s_2} \gets f_2(\out{{\tt entry}})$ \\\\
	$\out{s_3} \gets f_3(\out{s_2})$ \\\\
	$\out{s_4} \gets f_4(\out{s_3})$ \\\\
	$\out{s_5} \gets f_5(\out{s_4})$ \\\\
	$\out{s_6} \gets f_6(\out{s_5})$ \\\\
	$\out{s_7} \gets f_7(\out{s_6})$ \\\\
	$\out{s_8} \gets f_8(\out{s_7} \bigsqcap \out{s_{10}})$ \\\\
	$\out{s_9} \gets f_9(\out{s_8})$ \\\\
	$\out{s_{10}} \gets f_{10}(\out{s_9})$ \\\\
	$\out{s_{12}} \gets f_{12}(\out{s_8})$ \\\\
	$\out{{\tt Exit}} \gets \out{s_{12}}$ 
\end{tabular}


==> diagrams/block-diagram.tex <==

\hl{<placeholder for block diagram for whole system (static invariant generator and jit-c component)>}


==> diagrams/naive-composition.tex <==

	\[
		results(PTA)   
		\begin{cases}
		  OUT[l], \forall l \in \text{program-locations}
		\end{cases}
	\]


==> inlining-data-table.tex <==
\begin{figure}
	\small
\centering
\begin{tabular}{|l|l|c|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{ }}} 
& 
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Benchmark}}} 
& 
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\#monomorphic calls identified\end{tabular}}} 
& 
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\#inlining guards avoided\end{tabular}}}  \\
%&  
%\multicolumn{2}{c|}{\textbf{Artifact Size (KB)}} 
%& 
%\multicolumn{2}{c|}{\textbf{Overhead (\%)}} \\ \cline{5-8} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} &  &   \\ \hline
%\multicolumn{8}{|c|}{DaCapo 9.12-MR1-bach suite}\\\hline
1. & sunflow & 1862 & 1012 \\ 
2. & lusearch & 1860 & 1088  \\
3. & luindex & 2439 & 756  \\ 
4. & avrora & 3092 & 1396  \\
%\multicolumn{8}{|c|}{DaCapo 2006-10-MR2   suite}\\\hline
5. & antlr & 10524 & 8295   \\
6. & fop & 598 & 0   \\ 
7. & pmd & 5214 & 2579   \\  \hline
%6. & fop & 1.9 & 377 &  \multicolumn{1}{c|}{66} & 14 & \multicolumn{1}{c|}{3.39} & 0.719 \\ 
%7. & pmd & 2.0 & 2103 &  \multicolumn{1}{c|}{381} & 96 & \multicolumn{1}{c|}{18.60} & 4.68 \\ \hline
%\multicolumn{8}{|c|}{SPECjvm2008  suite}\\\hline
%8. & compress & 0.47 & 466 &  \multicolumn{1}{c|}{98} & 19 & \multicolumn{1}{c|}{20.40} & 3.96 \\ 
%9. & sparse & 0.47 & 480 &  \multicolumn{1}{c|}{93} & 18 & \multicolumn{1}{c|}{19.32} & 3.74 \\ 
%10. & sor & 0.47 & 480 &  \multicolumn{1}{c|}{94} & 18 & \multicolumn{1}{c|}{19.53} & 3.74 \\
%11. & fft & 0.47 & 485 &  \multicolumn{1}{c|}{94} & 18 & \multicolumn{1}{c|}{19.40} & 3.72 \\ 
%12. & montecarlo & 0.47 & 485 &  \multicolumn{1}{c|}{93} & 17 & \multicolumn{1}{c|}{19.40} & 3.54 \\ 
%13. & lu & 0.47 & 487 &  \multicolumn{1}{c|}{95} & 18 & \multicolumn{1}{c|}{19.66} & 3.72 \\ \hline
%\multicolumn{1}{|c}{}& geomean & 0.85 & 728 &  \multicolumn{1}{c|}{157.89} & 33.72 & \multicolumn{1}{c|}{18.02} & 3.85 \\ \hline
\end{tabular}
	\caption{Efficacy of using regenerated analysis results to
	identify monomorphic calls.}
	\label{fig:inlining-data-tab}
\end{figure} 


==> vpa-jitc-inter.tex <==
\subsection{Interprocedural EASY}

%\begin{figure}[t]
%	\centering
%	\input{algos/jitc-algo-inter}
%	\caption{Interprocedural EASY}
%\label{fig:easy-inter}
%\end{figure}


==> vpa-jitc-intra.tex <==
\subsection{Consumer in EASY: JIT Compiler}

%\begin{figure}[t]
%	\centering
%	\input{algos/jitc-algo-intra}
%	\caption{Intraprocedural EASY for methods with loops and recursive calls}
%\label{fig:easy-intra}
%\end{figure}
%The JIT compiler represents the subsequent stage -- $S_n$ -- where there is a need to perform points-to analysis efficiently.
%Attached to the JIT compiler is the ART verifier module whose responsibilities are twofold -- \begin{enumerate*} \item verify the safety of the ART instance -- $ART(PTA)$ -- transmitted by the static compiler \item use the safety-verified $ART(PTA)$ to regenerate the original whole-program flow-sensitive, context-insensitive points-to analysis -- $PTA$ -- efficiently. \end{enumerate*}
%The ART verifier module attached to the JIT compiler will handle these tasks, and make the regenerated $PTA$ available to future analyses and optimizations in the JIT compiler.
%
%
%Figure \ref{fig:easy-intra} presents the intraprocedural variant of EASY, which applies the ART technique to verify and regenerate $PTA$ for a single method. We will then extend this to the interprocedural dimension and show how to regenerate whole-program $PTA$.
%TODO:
%\begin{enumerate}
%  \item typeset the intraprocedural algorithm from the java points-to analysis perspective
%  \item explain the algorithm from method entry to exit, in simple terminology
%  \item extend the algorithm to the interprocedural dimension by using the callsite invariants as the ``glue''.
%\end{enumerate}


==> vpa-jitc-running.tex <==
%\subsection{Running Examples}
%We shall now apply this technique to the program snippets in Figure \ref{fig:motivating}.
%
%\subsubsection{Safety Verification in \textbf{EASY} in the presence of loops}
%
%%\begin{figure}[t]
%%  \centering
%%	\begin{subfigure}[t]{0.49\textwidth}
%%  	\includegraphics[width=\textwidth]{diagrams/loop-non-tampered.pdf}
%%	\caption{non-tampered ART, self-verified and safe to use}
%%	\label{fig:non-tampered}
%%	\end{subfigure}
%%	%\hspace{0.5em}
%%	\begin{subfigure}[t]{0.49\textwidth}
%%  	\includegraphics[width=\textwidth]{diagrams/loop-tampered.pdf}
%%	\caption{tampered ART}
%%	\label{fig:tampered}
%%	\end{subfigure}
%%
%%	\caption{Verification of ART for program in Figure \ref{fig:loop-motivating}}
%%	\label{fig:running-loop}
%%\end{figure}
%Figure \ref{fig:non-tampered} shows an example of an instance of ART from $S_{n-1}$ that is safe to use in $S_n$.
%$\mathcal{I}_{loop}[l_7]$ is assumed to be safe and is used as a drop-in for $\text{OUT}[l_7]$, then propagated over the control-flow path $l_8 \rightarrow l_9 \rightarrow l_7$.
%When $l_7$ is reached via the back-edge, we see that the invariant is unchanged.
%Hence proving that the safety-verified assumption was correct. Figure \ref{fig:tampered} shows an example of an ART that has been tampered.
%One of the edges denoting a heap reference in $\mathcal{I}_{loop}[l_7]$ is cut while transmitting the ART over the wire from $S_{n-1}$ to $S_n$.
%On propagating over the same control-flow path, we see that the $\text{IN}[l_7]$ has now changed.
%The removed edge is now re-discovered due to $l_8$.
%Thus, the assumption that $\mathcal{I}_{loop}[l_7]$ was an invariant, and thus safe to use, was wrong.
%
%\subsubsection{Safety Verification in \textbf{EASY} in the presence of recursion}
%\begin{figure}[t]
%	\centering
%  	\includegraphics[width=\textwidth]{diagrams/rec-tampered.pdf}
%	\caption{Verification of ART for program in Figure \ref{fig:rec-motivating}}
%	\label{fig:rec-tampered}
%\end{figure}
%Figure \ref{fig:rec-tampered} shows an instance of ART for the program in Figure \ref{fig:rec-motivating}.
%$\mathcal{I}_{out}[\texttt{foo}]$ has been tampered with to remove one of the heap reference edges.
%At location $l_{12}$, $\mathcal{I}_{out}[\texttt{foo}]$ is projected back to the call site.
%However the missing heap reference edge has already been discovered due to location $l_{11}$.
%The resultant $\text{out-summary}[\texttt{foo}]$ is thus not the same as $\mathcal{I}_{out}[\texttt{foo}]$.
%This implies that the ART is not in sync with the program being analyzed by $S_n$, thus indicating tampering.


==> vpa-jitc.tex <==
\subsection{JIT Compilation part of EASY}
\input{algos/jitc-algo-a}

	%- Build the Points-to graph
The responsibility of the JIT compilation stage of EASY is twofold -- \begin{enumerate*} \item verify the safety of each type of invariant transmitted by the static compilation stage \item use these safety-verified invariants to re-generate (\hl{re-compute?}) the original whole-program flow-sensitive, context-insensitive points-to analysis efficiently. \end{enumerate*}
We will first present the intuition behind verifying the safety of each type of invariant, followed by an algorithm that builds the whole-program points-to analysis.
\subsubsection{Intuition behind safety verification}

\hl{\textbf{Note to Self:} following passage is meant to be an intuition. So we haven't introduced the \textit{subsumes} operator yet.}
\begin{enumerate}
  \item \textbf{Loop-Invariants:}
    Recall that a \textit{loop-invariant} is the fixpoint points-to graph at a loop header captured after termination of points-to analysis in the static compilation stage.
    Computation of this data-flow value involved analyzing the program statements in the body of the corresponding loop repeatedly until the data-flow value at the loop header stabilized -- i.e. reached fixpoint.
    Any further analysis of the body of the loop results in no change to the data-flow value at the loop header.
    We can leverage this property to verify that a loop-invariant transmitted to the JIT compilation stage is truly an un-tampered invariant.
    \hl{At this point, shouldn't there be a discussion on safe (conservative/additive) tampering and unsafe (reductive) tampering?}
    If $l_h$ is the program location corresponding to a loop header, the untampered loop-invariant is given by $G = \mathcal{I}_{loop}[l_h]$.
    We denote an unsafe tampering of the loop invariant at $l_h$ as follows: ${\mathcal{I}_{loop}}^\prime  : \mathcal{I}_{loop}[l_h] \leftarrow G \setminus {g}$, where ${g}$ represents a subset of the points-to graph $G$.
    Now consider $G = \mathcal{I}_{loop}[l_h]$  and $G^\prime = {\mathcal{I}_{loop}}^\prime[l_h]$.
    Let the operation $\xrightarrow{\text{1 iter}}$ represent the action of propagating the invariant over the loop body for one more iteration.
    without any assumptions about safety, if we propagate both $G$ and $G^\prime$ over the loop body for one more iteration, following will the result -- $G \xrightarrow{\text{1 iter}} G$ and $G^\prime \xrightarrow{\text{1 iter}} G^{\prime\prime}$
    Propagating $G^\prime$ over the loop body will result in a new points-to graph $G^{\prime\prime}$ while doing so for $G$ results in the same points-to graph $G$.
    We use this intuition as a verification condition for loop invariants - 
    \begin{enumerate}
      \item if a loop invariant transmitted to the JIT compilation stage is a fixpoint points-to graph, propagating it over the loop body for one iteration will result in no change to the points-to graph at the loop header. This provides a guarantee that the loop-invariant is the fixpoint points-to graph corresponding to the loop header in the bytecode being analyzed by the JIT compiler, and thus, is safe to use.
      \item if a loop-invariant transmitted to the JIT compilation stage has been unsafely tampered, propagating it over the loop body for one iteration will result in a change to the points-to graph at the loop header -- thus proving tampering.
    \end{enumerate}
  \item \textbf{Out-Invariants:}
    The out-invariants are intended to replace the fixpoint computation of the out-summary of a recursively invoked method.
    On encountering a call site where the call is recursive (\hl{how will it know? is there a standard algorithm to cite?}) -- the JIT compilation stage will assume that the provided out-invariant for the callee is verified, and proceed to use it as a drop-in data-flow value for that call site, and proceed with analyzing the rest of the program statements of the caller in control-flow order.
    Then, when the algorithm reaches the tail of the caller's control-flow graph (\hl{or should we just say exit of the method}), it checks to see if the out-summary just computed is the same as the out-summary that was dropped-in at the recursive call site.
    i.e. let $M_{\text{rec}}$ be a recursive method, $\mathcal{I}_{out}[M_{\text{rec}}]$ the statically computed out-summary for $M_{\text{rec}}$.
    Let $G_{\text{out}}$ be the JIT compiler computed out-summary of $M_{\text{rec}}$.
    Then, if $\mathcal{I}_{out}[M_{\text{rec}}] \equiv G_{\text{out}}$ -- then the assumption that the out-summary that was dropped in at the recursive call site is verified was in fact a right assumption.
  \item \textbf{In-Invariants:}
\end{enumerate}




==> vpa-static.tex <==
\subsection{Producer in EASY: Static Analyzer}
%EASY maps $S_{n-1}$ to the Java static compiler housing a flow-sensitive, context-insensitive points-to analysis (\hl{which form of points-to analysis? insert citation here}). We denote this points-to analysis by $PTA$.
%
%The components of ART described in Section \ref{s:art-composition} translate directly to Java points-to analysis and the constituent invariants of ART -- loop-invariants, out-invariants and in-invariants -- all hold the same connotation.
%Once $PTA$ reaches termination, the ART encoder module will intercept the results and dump the necessary points-to graphs as prescribed by ART for points-to analysis, as $ART(PTA)$.



==> vpa.tex <==
%\section{Verified Points-to Analysis}

\subsection{ART for Points-to-Analysis of Java Programs}
%\label{l:vpa}
%\begin{figure}[t]
%	\centering
%  \includegraphics[width=\textwidth]{diagrams/block-easy.pdf}
%  \caption{Implementation of EASY with respect to points-to analysis of Java programs}
%	\label{fig:block-easy}
%\end{figure}
\begin{figure}[t]
	\small
	\centering
  \includegraphics[scale=0.7]{diagrams/block-easy.pdf}
  \caption{Adapting ART for points-to analysis of Java programs.}
	\label{fig:block-easy}
\end{figure}
The proposed scheme of ART can be adapted to any pair of compilation
stages in a multi-stage compilation system, where there exists a need to
perform expensive points-to analysis in one stage and transmit the results
for use (after establishing safety) in a subsequent stage.
In this section, we will adapt ART to Java, where the consumer (the JIT compiler or a program analysis tool) can obtain precise
points-to analysis information by using the \artwork{} (after
establishing its safety) generated during static analysis/compilation.

Fig. \ref{fig:block-easy} shows how the idea of ART can be incorporated
into the multi-stage Java compilation system.
Producer: The static java compiler (for example, {\tt javac}), which can have a
static analyzer component, will take a Java
application as input and emit the \artwork{} generated by the static
analyzer, along with the bytecode.
Alternatively, we can envisage a static analyzer 
framework that takes compiled Java
bytecode (for example, {\tt .class} files) as input and emits the
\artwork{} for the input bytecode.
In both cases, the static analyzer will invoke the points-to analyzer
(PTA) and generate the \artwork{}.
Consumer: A program analysis tool, or the JIT compiler (invoked by the Java Virtual
Machine at runtime) will invoke the ART regenerator to establish the safety of the
given \artwork{}  and regenerate the original results
obtained by the static PTA for the input bytecode.

In case the regenerator deduces that the input \artwork{} is tampered with (and
hence unsafe to use, see Sections~\ref{ss:art-intra-safety}
and~\ref{ss:art-inter-safety}) then there are two possible paths it can
take: (i)~it can throw an error  and abort the JIT
compilation or analysis being performed by the consumer, or~(ii) give a warning, discard
all the regenerated points-to analysis results and continue
the JIT compilation or analysis like it would in the absence of our technique.
For simplicity, we stick to the option~(i).
One can also envisage some more strategies between the two paths;
such an exploration is beyond the scope of our current manuscript, and we
leave it as an interesting future work.

%> Given a specific flow-sensitive context-insensitive iterated-dataflow analysis (including details like transfer functions, lattice, handling method calls etc) then to implement it using ART, we need to address the following:
%>
%> *  identify the representation of the data-flow values (e.g., points-to graph for points-to analysis, or variables-to-constant maps for constant propagation, variables-to-taint-status map in case of taint analysis) and the subsumes operator. Recall that given two data-flow values I1 and I2, the subsumes operator can be used to check if I1 subsumes I2 (for example, see Section 2, last paragraph).
%> * implement a producer component that dumps ARTWORK (Sections 3.1 and 3.4) specific to the analysis under consideration.
%> * implement a consumer that reads the ARTWORK and invokes the regenerate function (Section 3.5).
%> 
%> As it can be seen these steps are mainly implementation details specific to each analysis and do not need extending the core idea of ART and the underlying safety argument
%

%It consists of two compilation stages -- the static compiler and JIT compiler of Java -- and a pair of ART encoder-verifier modules that assist in encoding and verifying the ART artifacts, regenerating the original points-to analysis and making it available for use in the later passes of the JIT compiler.

%\input{vpa-static}
%\input{vpa-jitc-intra}

%\subsection{Correctness argument}

%\input{vpa-jitc-running}
%\input{vpa-jitc-inter}

